Identity-Consistent Multi-Pose Generation of Contactless Fingerprints

Contactless fingerprint recognition has gained increasing attention due to its advantages in hygiene and acquisition flexibility. However, the absence of physical contact constraints introduces severe nonlinear geometric distortions caused by free finger poses in 3D space, resulting in a substantial cross-modal domain gap between contactless and conventional contact-based fingerprints. Existing solutions largely rely on explicit geometric correction or image enhancement, which are fragile under extreme pose variations. In this paper, we propose Identity-Consistent Multi-Pose Generation of Contactless Fingerprints (IMPOSE), a physics-inspired framework that synthesizes identity-preserving, multi-pose contactless fingerprint samples to empower recognition models. IMPOSE consists of three stages: (1) rolled fingerprint identity generation via latent diffusion with discrete codebook representations, (2) cross-modal translation from rolled to contactless modality guided by Sauvola-based local adaptive binarization as an identity anchor, and (3) physics-based multi-pose simulation through 3D finger model texture mapping and projection. The generated samples maintain strict identity consistency at the ridge topology level and spatial alignment with standard fingerprint coordinate space. Extensive experiments on the UWA and PolyU CL2CB databases demonstrate that fine-tuning fixed-length dense descriptors (FDD) with IMPOSE-synthesized data achieves state-of-the-art cross-modal matching, reducing EER to 8.74% on UWA and 2.26% on PolyU CL2CB. Synthetic data also yields consistent gains across mainstream representations including DeepPrint and AFRNet, and the hybrid strategy combining synthetic and real data achieves the best overall results. The code and generated samples are available at https://github.com/Yu-Yy/IMPOSE.

==> macros/revision_macros.tex <==
% Shared switch: normal entry points are black; *_blue.tex sets the flag.
\RequirePackage{xcolor}
% Table contents, captions, and notes stay black in both output variants.
\newif\ifIMPOSEBlackTable
\newcommand{\revisioncolor}{%
  \ifIMPOSEBlackTable\color{black}%
  \else\ifdefined\IMPOSEBlueChanges\color{blue}\fi\fi}
\newcommand{\blacktable}{\IMPOSEBlackTabletrue\color{black}}
\DeclareRobustCommand{\rev}[1]{\begingroup
  \revisioncolor
  #1\endgroup}
\newenvironment{revision}{\begingroup
  \ifdefined\IMPOSEBlueChanges\color{blue}\fi}{\endgroup}
% Used inside changed floats, after IEEEtran has reset their font and color.
\newcommand{\revisionfloatcolor}{\revisioncolor}
% Main text and supplement now share one document, so cross-part references
% resolve directly; the two entry points are kept for source readability.
\newcommand{\suppref}[1]{\ref{#1}}
\newcommand{\mainref}[1]{\ref{#1}}

